Fast Rates for Empirical Risk Minimization of Strict Saddle Problems

We derive bounds on the sample complexity of empirical risk minimization (ERM) in the context of minimizing non-convex risks that admit the strict saddle property. Recent progress in non-convex optimization has yielded efficient algorithms for minimizing such functions. Our results imply that these efficient algorithms are statistically stable and also generalize well. In particular, we derive fast rates which resemble the bounds that are often attained in the strongly convex setting. We specify our bounds to Principal Component Analysis and Independent Component Analysis. Our results and techniques may pave the way for statistical analyses of additional strict saddle problems.

==> header.tex <==
% \usepackage{graphicx}
% \usepackage{epsfig}
% \usepackage{hyperref}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{algorithm}
% \usepackage{algorithmic}
% \usepackage{array}
% \usepackage{eqparbox}
% \usepackage{url}
% \usepackage{enumerate}
% \usepackage{amsfonts}
% \usepackage{boxedminipage}
% \usepackage{xcolor}
%  \usepackage{framed}  
% \usepackage{rotating}
% \usepackage{array}
% \usepackage{multirow}
% \usepackage{color}
% \usepackage{tikz}
% \usepackage{pgfplots}
% \usepackage{mathabx}
% \usepackage{tabularx,ragged2e,booktabs,caption}



% algorithms
x% \newenvironment{myalgo}[1]%
% {
% %\vspace{0.3cm}
% \begin{center}
% \begin{boxedminipage}{0.8\linewidth}
% \begin{center}
% \textbf{\texttt{#1}}
% \end{center}
% \rm
% \begin{tabbing}
% ....\=...\=...\=...\=...\=  \+ \kill
% } %
% {\end{tabbing} 
% \end{boxedminipage} \end{center} %\vspace{0.3cm}
% }

% \renewcommand\algorithmiccomment[1]{%
%   \hfill\#\ \eqparbox{COMMENT}{#1}%
% }


% \newenvironment{myrule}[1]%
% {
% \vspace{0.01cm}
% \begin{center}
% \begin{boxedminipage}{0.8\linewidth}
% \begin{center}
% \textbf{\texttt{#1}}
% \end{center}
% } %
% {
% \end{boxedminipage} \end{center} \vspace{0.3cm}
% }


% theorems with small letters
% \newtheorem{definition}{Definition}
% \newtheorem{lemma}{Lemma}
% \newtheorem{corollary}{Corollary}
% \newtheorem{theorem}{Theorem}
% \newtheorem{proposition}{Proposition}
% \newtheorem{assumption}{Assumption}
% \newtheorem{example}{Example}
% \newtheorem{exercise}{Exercise}
% \newtheorem{solution}{Solution}
% \newtheorem{remark}{Remark}
% \newtheorem{claim}{Claim}

% bf - letters
\newcommand{\bx}{{\mathbf x}}
\newcommand{\by}{{\mathbf y}}
\newcommand{\bz}{{\mathbf z}}
\newcommand{\bw}{{\mathbf w}}
\newcommand{\bv}{{\mathbf v}}
\newcommand{\bu}{{\mathbf u}}
\newcommand{\be}{{\mathbf e}}
\newcommand{\br}{{\mathbf{r}}}
\newcommand{\bsig}{{\mathbf \sigma}}

%bf - numbers
\newcommand{\bzero}{{\mathbf{0}}}

% bf - expressions
\newcommand{\rV}{{\mathbf {Var}}}


% mathbb
\newcommand{\prob}{\mathbb{P}}
\newcommand{\bE}{\mathbb{E}}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\realspsd}{\mathbb{R}_{+}}
\newcommand{\realspd}{\mathbb{R}_{++}}
\newcommand{\realsnsd}{\mathbb{R}_{-}}
\newcommand{\realsnd}{\mathbb{R}_{--}}
\newcommand{\bN}{\mathbb{N}}
\newcommand{\bZ}{\mathbb{Z}}
\newcommand{\bC}{\mathbb{C}}
\newcommand{\bQ}{\mathbb{Q}}
\newcommand{\bB}{\mathbb{B}}
\newcommand{\bF}{\mathbb{F}}

% bars
\newcommand{\barw}{\bar{\w}}
\newcommand{\barF}{\bar{F}}
\newcommand{\barlambda}{\bar{\lambda}}
\newcommand{\barA}{\bar{A}}
\newcommand{\barI}{\bar{I}}

%mathrm
\newcommand{\sgn}{{\mathrm{sgn}}}
\newcommand{\rank}{\mathrm{rank}}
\newcommand{\supp}{\mathrm{supp}}
\newcommand{\spn}{\mathrm{span}}
\renewcommand{\Im}{\mathrm{Im}}
\newcommand{\diag}{{\mathrm{diag}}}
\newcommand{\T}{\mathrm{time}}
\newcommand{\sig}{\mathrm{sig}}
\newcommand{\poly}{\mathrm{poly}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\thalf}{\tfrac{1}{2}}
\newcommand{\eqdef}{\stackrel{\mathrm{def}}{=}}
\newcommand{\opt}{\mathrm{opt}}
\newcommand{\Var}{\mathrm{Var}}


%tildes and hats
\newcommand{\tu}{\tilde{u}}
\newcommand{\tv}{\tilde{v}}
\newcommand{\tw}{\tilde{w}}
\newcommand{\tsig}{\tilde{\sigma}}
\newcommand{\tx}{\tilde{x}}
\newcommand{\tz}{\tilde{z}}
\newcommand{\tU}{\tilde{U}}
\newcommand{\tV}{\tilde{V}}
\newcommand{\tA}{\tilde{A}}
\newcommand{\tX}{\tilde{X}}
\newcommand{\tSig}{\tilde{\Sigma}}
\newcommand{\tL}{\tilde{L}}
\newcommand{\tg}{\tilde{g}}
\newcommand{\tH}{\tilde{H}}
\newcommand{\tf}{\tilde{f}}

% hats
\newcommand{\hu}{\hat{u}}
\newcommand{\hv}{\hat{v}}
\newcommand{\hw}{\hat{w}}
\newcommand{\hsig}{\hat{\sigma}}
\newcommand{\hx}{\hat{x}}
\newcommand{\hz}{\hat{z}}
\newcommand{\hU}{\hat{U}}
\newcommand{\hV}{\hat{V}}
\newcommand{\hg}{\hat{g}}
\newcommand{\hH}{\hat{H}}
\newcommand{\hSig}{\hat{\Sigma}}
\newcommand{\hf}{\hat{f}}
\newcommand{\hF}{\hat{F}}


%  mathcal
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cT}{\mathcal{T}}

% miscellaneous
\newcommand{\mathcomment}[1]{\color{red}{\textbf{#1}}}
\newenvironment{proof}{\par\noindent{\bf Proof\ }}{\hfill\BlackBox\\[2mm]}
\newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  
\newcommand{\overbar}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}
\newcommand{\alon}[1]{\footnote{#1 (alon)}}
\newcommand{\todo}[1]{{\color{red}\bf TODO: #1}}
\newcommand{\thought}[1]{\footnote{{\color{blue} \bf Thought: #1}}}
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}




% disjoint union
\makeatletter
\def\moverlay{\mathpalette\mov@rlay}
\def\mov@rlay#1#2{\leavevmode\vtop{%
   \baselineskip\z@skip \lineskiplimit-\maxdimen
   \ialign{\hfil$\m@th#1##$\hfil\cr#2\crcr}}}
\newcommand{\charfusion}[3][\mathord]{
    #1{\ifx#1\mathop\vphantom{#2}\fi
        \mathpalette\mov@rlay{#2\cr#3}
      }
    \ifx#1\mathop\expandafter\displaylimits\fi}
\makeatother
\newcommand{\cupdot}{\charfusion[\mathbin]{\cup}{\cdot}}
\newcommand{\bigcupdot}{\charfusion[\mathop]{\bigcup}{\cdot}}

% machine learning
\newcommand{\LZO}{\ell^{0-1}}
\newcommand{\LH}{\ell^{\text{hinge}}} 
\newcommand{\LD}{L_{\cD}}
\newcommand{\LDZO}{L_{\cD}^{0-1}} 
\newcommand{\LDH}{L_{\cD}^{\text{hinge}}} 
\newcommand{\VC}{\mathrm{VCdim}}
\newcommand{\regret}{\textrm{Regret}}
\newcommand{\hL}{\hat{L}}

% Real Analysis
\newcommand{\ballr}[3]{B_#1 ^#2 (#3)}   % 1-dimension, 2-norm, 3-radius
\newcommand{\ball}[2]{B_#1 ^#2}   % same with radius 1
\newcommand{\inter}{\mathrm{int}}
\newcommand{\cl}{\mathrm{cl}}
\newcommand{\bd}{\mathrm{bd}}
\newcommand{\limn}{\lim_{n \rightarrow \infty}} 
\newcommand{\IFF}{\Leftrightarrow}
\newcommand{\indct}[1]{\boldsymbol{1}\!_{\left[ #1 \right]}}
\newcommand{\vol}{\mathrm{vol}}
\newcommand{\embeds}[1]{\overset{#1}{\hookrightarrow}}
\newcommand{\aff}{\mathrm{aff}}
\newcommand{\id}{\mathrm{id}}

% Convex Analysis
\newcommand{\conv}{\textrm{conv}}

% Linear Algebra
\newcommand{\sym}[1]{\mathbb{S}^{#1}}
\newcommand{\symps}[1]{\mathbb{S}^{#1}_{+}}
\newcommand{\symp}[1]{\mathbb{S}^{#1}_{++}}
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\vect}{\mathrm{vec}}
\newcommand{\trans}{\dagger}
\newcommand{\inner}[1]{\langle #1 \rangle}
\newcommand{\finner}[1]{\langle #1 \rangle_F}
\newcommand{\fnorm}[1]{\| #1\|_F}
\newcommand{\snorm}[1]{\| #1\|_{\mathrm{sp}}}
\newcommand{\tnorm}[1]{\| #1\|_{\mathrm{tr}}}
\newcommand{\twonorm}[1]{\| #1\|_2}
\newcommand{\onenorm}[1]{\| #1\|_1}
\newcommand{\infnorm}[1]{\| #1\|_\infty}
\newcommand{\dnorm}[1]{\| #1\|_\star}
\newcommand{\image}{\mathrm{Im}}
\newcommand{\nnz}{\mathrm{nnz}}


%boldsymbol
\newcommand{\vtheta}{\boldsymbol{\theta}}
%\newcommand{\tw}{\tilde{w}}






%DeclareMath
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max} 
\DeclareMathOperator*{\arginf}{arg\,inf} 
\DeclareMathOperator*{\argsup}{arg\,sup} 
\DeclareMathOperator{\Span}{span}


% ref
\renewcommand{\eqref}[1]{Equation~(\ref{#1})}
\newcommand{\exref}[1]{Example~(\ref{#1})}
\newcommand{\exeref}[1]{Exercise~(\ref{#1})}
\newcommand{\figref}[1]{Figure~\ref{#1}}
\newcommand{\secref}[1]{Section~\ref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}
\newcommand{\appref}[1]{Appendix~\ref{#1}}
\newcommand{\thmref}[1]{Theorem~\ref{#1}}
\newcommand{\lemref}[1]{Lemma~\ref{#1}}
\newcommand{\defref}[1]{Definition~\ref{#1}}
\newcommand{\corref}[1]{Corollary~\ref{#1}}
\newcommand{\clref}[1]{Claim~\ref{#1}}
\newcommand{\algref}[1]{Algorithm~\ref{#1}}
\newcommand{\chapref}[1]{Chapter~\ref{#1}}
\newcommand{\remref}[1]{Remark~\ref{#1}}
\newcommand{\assref}[1]{Assumption~\ref{#1}}




% % handouts

% \newcommand{\coursename}{(67577) INTRODUCTION TO MACHINE LEARNING}

% \hbadness=10000
% \vbadness=10000

% \setlength{\oddsidemargin}{.25in}
% \setlength{\evensidemargin}{.25in}
% \setlength{\textwidth}{6in}
% \setlength{\topmargin}{-0.4in}
% \setlength{\textheight}{8.5in}

% \newcommand{\handout}[5]{
%    \renewcommand{\thepage}{#1-\arabic{page}}
%    \noindent
%    \begin{center}
%    \framebox{
%       \vbox{
%     \hbox to 5.78in { {\bf (67577) Introduction to Machine Learning}
%          \hfill #2 }
%        \vspace{4mm}
%        \hbox to 5.78in { {\Large \hfill #5  \hfill} }
%        \vspace{2mm}
%        \hbox to 5.78in { {\it #3 \hfill #4} }
%       }
%    }
%    \end{center}
%    \vspace*{4mm}
% }

% % lecture
% \newcommand{\lecture}[4]{\handout{#1}{#2}{Lecturer:
% #3}{Scribe: #4}{Lecture #1}}

% % New exercise
% \newcommand{\problemset}[2]{\handout{#1}{}{}{Due: #2}{Exercise #1}}
% % usage: \problemset{1}{\today}

% % School solution
% \newcommand{\schoolSolution}[2]{\handout{#1}{}{Written by:
%     #2}{}{Problem Set #1 - Solution}}
% % usage: \schoolSolution{1}{Alon}

% % Submitted solution
% \newcommand{\exanswer}[2]{\handout{#1}{}{by: #2}{}{Problem Set #1 -
%     Answers}}
%usage: \exanswer{1}{Alon}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:

